Data-driven Verification of Procedural Programs with Integer Arrays

We address the problem of verifying automatically procedural programs manipulating parametric-size arrays of integers, encoded as a constrained Horn clauses solving problem. We propose a new algorithmic method for synthesizing loop invariants and procedure pre/post-conditions represented as universally quantified first-order formulas constraining the array elements and program variables. We adopt a data-driven approach that extends the decision tree Horn-ICE framework to handle arrays. We provide a powerful learning technique based on reducing a complex classification problem of vectors of integer arrays to a simpler classification problem of vectors of integers. The obtained classifier is generalized to get universally quantified invariants and procedure pre/post-conditions. We have implemented our method and shown its efficiency and competitiveness w.r.t. state-of-the-art tools on a significant benchmark.

==> chc-and-solving.tex <==
\section{Constrained Horn Clauses (CHC) and CHC solving}
\label{sec:chc-and-solving}

\ssubsubsection{Constrained Horn Clauses}
\label{subsec:chc}
Here, we present constrained Horn clauses as a formal representation to encode the verification conditions (VCs) associated with the program under verification. %If the system of CHC derived from a program and its specification is satisfiable, then the program does indeed satisfy its specification.
In general CHC can be over any first-order logical
theory $\mathcal{T}$.
In our case, we will use the array logic defined
previously.

\begin{definition}
Let $\mathcal{P}$ be a set of uninterpreted predicate/relation symbols.
A \emph{constrained Horn clause} (CHC) is a formula in
some first-order theory $\mathcal{T}$
that has one of the three forms
\begin{align*}
\forall \vec{v}.\; \phi(\vec{v}) & \implies \Predicate{P}(\vec{v}) \\
\forall \vec{v}_1,\dots,\vec{v}_n,\vec{v}.\; \Predicate{P_1}(\vec{v}_1) \land \dots \land \Predicate{P_n}(\vec{v}_n) \land \phi(\vec{v}_1,\dots,\vec{v}_n, \vec{v}) & \implies \Predicate{P}(\vec{v}) \\
\forall \vec{v}_1,\dots,\vec{v}_n.\; \Predicate{P_1}(\vec{v}_1) \land \dots \land \Predicate{P_n}(\vec{v}_n) \land \phi(\vec{v}_1,\dots,\vec{v}_n) & \implies \bot
\end{align*}
where $\Predicate{P_1},\dots,\Predicate{P_n} \in \mathcal{P}$ and $\Predicate{P} \in \mathcal{P}$ are not necessarily distinct uninterpreted predicate symbols with vectors of variables $\vec{v}_1$, $\dots$, $\vec{v}_n$ and $\vec{v}$ respectively as parameters. The $\phi$ are formulas
%\footnote{All function and relation symbols are interpreted within $\mathcal{T}$.}
with designated free variables. %in $\vec{v}_1$, $\dots$, $\vec{v}_n$ and possibly $\vec{v}$.
\end{definition}

\begin{definition}\label{def:chc-satisfiable}
Given a set of uninterpreted predicate symbols $\mathcal{P}$ and a set of constraint Horn clauses $H$ over $\mathcal{P}$, $H$ is \emph{satisfiable} if there exists an interpretation which assigns to each $k$-ary symbol in $\mathcal{P}$ a relation over $k$ tuples such that all clauses in $H$ are valid.
\end{definition}

A constrained Horn clauses problem is to determine satisfiability of a set of CHCs $H$.
Later, we are looking for a particular
\emph{solution} of the CHC problem where
to each $k$-ary symbol in $\mathcal{P}$ a
parametric-size array properties with $k$ free variables
is associated which realizes the interpretation in the definition above.

%\ssubsubsection{Safety verification as CHC solving}
%Safety verification of a given program with its specification can be reduced as described in \cite{chc-for-verification-1,chc-for-verification-2} to solving a constrained Horn clauses problem over uninterpreted predicate symbols.

%We sketch this briefly.
%To each loop in the program we associate 
%an uninterpreted predicate, representing its invariant.
%This uninterpreted predicate is defined over the variables declared at the loop's location.
%Additionally, to every procedure (excluding \texttt{main}) two uninterpreted predicates are associated: one representing its precondition, defined over the parameters of the procedure, and the other representing its postcondition, defined over both the parameters and the return value of the procedure.
%If the procedure modifies the content of one of its array pointer parameters\footnote{We use pass-by-value semantics for arrays passed to procedures through pointers.}, the postcondition's predicate is also over the value of the modified array at the procedure return point(s).
%%The derived CHC are over the %parametric-size
%%array theory.
%If the program has no procedures, these CHC are linear; otherwise, they are non-linear.
%If the derived CHC are satisfiable (see Def.~\ref{def:chc-satisfiable}) then the program is \emph{safe}; otherwise, we may find a finite trace that shows that it does not satisfy its specification.
%We aim for an approach that is not restricted to only checking if the CHC are satisfiable but also able to infer formulas for the uninterpreted predicates satisfying the clauses as they represent invariants and procedures' pre/post-conditions that may be useful for the user.%

%The loop invariant $\Predicate{I}$ of a loop over variables $\vec{v}$ with a condition $b(\vec{v})$ is required to (1) include its precondition $\forall \vec{v}.\; Pre(\vec{v}) \implies \Predicate{I}(\vec{v})$, (2) imply its postcondition upon exiting the loop $\forall \vec{v}.\; \Predicate{I}(\vec{v}) \land \neg b(\vec{v}) \implies Post(\vec{v})$, and (3) it is inductive $\forall \vec{v}, \vec{v}'.\; \Predicate{I}(\vec{v}) \land b(\vec{v}) \land Trans(\vec{v}, \vec{v}') \implies \Predicate{I}(\vec{v}')$, where $Trans(\vec{v}, \vec{v}')$ encodes the transition by the body of the loop.
%When a program has a complicated control structure (e.g., multiple loops, nested loops, procedure calls...), the precondition and postcondition of a loop in that program may be defined in terms of other loops' invariants and/or procedures' pre/post-conditions.%

%A procedure definition is translated into Horn clauses using its precondition that must be satisfied at the procedure's entry, and its postcondition over its inputs and results that must be satisfied after executing its body.
%Every procedure call is captured by a Horn clause stating that the precondition of the call location must satisfy the procedure's precondition, and another clause stating that if the procedure's precondition holds and the inputs and output of the call satisfy its postcondition, then the postcondition of the call position also holds.

To summarize, from a program we obtain a CHC problem with uninterpreted predicates $\mathcal{P}$ over our array logic $\BoundedArrayTheory{A}{}$ whose formulas $\phi$ are not restricted to a particular fragment.
However, we are looking for a solution where all uninterpreted predicates
are parametric-size array properties.
Checking that such a solution is correct is undecidable in general, but for almost all considered programs, the $\phi$'s are such that it is decidable.
For an uninterpreted predicate $\Predicate{P} \in \mathcal{P}$, let $\VariablesOf{\Predicate{P}}$ denote the set of all its variable parameters, $\ArraysOf{\Predicate{P}} \subseteq \VariablesOf{\Predicate{P}}$ be the set of its arrays, $\VariablesTypedOf{\Predicate{P}}{\B} \subseteq \VariablesOf{\Predicate{P}}$ the set of its boolean variables, $\VariablesTypedOf{\Predicate{P}}{idx} \subseteq \VariablesOf{\Predicate{P}}$ the set of its integer variables referring to index integer variables in $V_{idx}$ and $\VariablesTypedOf{\Predicate{P}}{data} \subseteq \VariablesOf{\Predicate{P}}$ the set of its integer variables referring to data integer variables in $V_{data}$.


==> horn-ice.tex <==
\section{Data-driven CHC solving using Horn-ICE}
\label{section:horn-ice}

To solve the CHC problem generated by the previous step, our method instantiates the Horn-ICE framework \cite{horn-ice}
defined over an arbitrary background logic $\mathcal{T}$.
We briefly describe it here.
Horn-ICE uses the active learning paradigm to solve a system of CHC by extending the ICE learning
framework \cite{ice}. It comprises an iteratively communicating learner and teacher, as shown in Fig.~\ref{fig-algo:horn-ice}.

\begin{figure*}[ht]
 % \scriptsize
  \centering
  \begin{minipage}{.8\linewidth}
    \begin{algorithm}[H]
      \SetKwInOut{Input}{Input}
      \SetKwInOut{Output}{Output}
    
      \Input{A CHC system $H$ in $\mathcal{T}$ over predicates $\mathcal{P}$}
      \Output{A solution for $H$ or \texttt{UNSAT}}
      Initialize Horn-ICE sample $\mathcal{S}=(X, C) \gets (\emptyset, \emptyset)$\;
      \While{true}{
        $J \gets \textsc{Learner.learn}(\mathcal{S})$\;\label{hornice:line:learn}
        $(success,counterexample) \gets \textsc{Teacher.is\_solution}(J)$\;\label{hornice:line:check}
        \If{$success$}{
          \KwRet{$J$}\;
        } \Else {
          $S \gets \textsc{add}(S, counterexample)$\;\label{hornice:line:addce}
          \If{$S$ is inconsistent}{
            \KwRet{\texttt{UNSAT}}\;
          }
        }
      }
    \end{algorithm}
  \end{minipage}
  %\setlength{\abovecaptionskip}{0ex}
  %\setlength{\belowcaptionskip}{-5ex}
  \caption{The main loop of {Horn-ICE}.}\label{fig-algo:horn-ice}
\end{figure*}

In every iteration, the learner, agnostic of the CHC, synthesizes a candidate solution $J$ in line~\ref{hornice:line:learn}.
It associates to each uninterpreted
predicate in $\mathcal{P}$ a formula in
the background logic by considering a \emph{Horn-ICE sample}
$\mathcal{S} = (X, C)$ where $X$ is a set of data points
and $C$ a set of Horn implications over $X$.
Intuitively a \emph{data point} $x \in X$ corresponds to a configuration of
the program at some location or input/output configurations for a postcondition.
To each data point is associated an uninterpreted predicate $\Predicate{P} \in \mathcal{P}$ (denoted by $\PredicateOfDatapoint{x}$)
and a vector of constants of the logic $\mathcal{T}$
with an entry for each parameter variable of $\Predicate{P}$.
A \emph{Horn implication} over $X$ is a hyperedge (generalizing ICE's implication) of the forms:
%\begin{itemize}
%\item
(a) $\top \rightarrow x$, where $x \in X$, meaning $x$ should satisfy
  the predicate $\PredicateOfDatapoint{x}$;
(b) $x_1 \land  \dots \land x_n \rightarrow x$, where $x_1,\dots,x_n,x \in X$, i.e. if $x_1,\dots,x_n$, respectively, satisfies $\PredicateOfDatapoint{x_1},\dots,\PredicateOfDatapoint{x_n}$ then $x$ should satisfy $\PredicateOfDatapoint{x}$, or if $x$ doesn't satisfy $\PredicateOfDatapoint{x}$ at least one of the $x_1,\dots,x_n$ should not satisfy its predicate;
(c) $x_1 \land  \dots \land x_n \rightarrow \bot$, where $x_1,\dots,x_n \in X$,  i.e. at least one of the $x_1,\dots,x_n$ should not satisfy its predicate.
For a sample $\mathcal{S} = (X, C)$, we define inductively $\mathcal{S}^+$
(resp. $\mathcal{S}^-$), the set of data points that must (not)
satisfy their respective predicates.

{\small
\begin{eqnarray}
\forall \top \rightarrow x \in C.\; x \in \mathcal{S}^+ \label{eq:cs:1} \\
\forall x \rightarrow \bot \in C.\; x \in \mathcal{S}^- \\
\forall x_1 \land \dots \land x_n \rightarrow x \in C.\; x_1,\dots,x_n \in \mathcal{S}^+ \implies x \in \mathcal{S}^+ \\
\forall x_1 \land  \dots \land x_n \rightarrow x \in C.\; x_1,\dots,x_{i-1},x_{i+1},\dots,x_n \in \mathcal{S}^+ \land x \in \mathcal{S}^- \implies x_i \in \mathcal{S}^- \label{eq:cs:4}
\end{eqnarray}}
Initially, the sample is empty.
The candidate solution $J$ synthesized by the learner is assumed to be \emph{consistent} with the sample, i.e. data points in $\mathcal{S}^+$ satisfy their respective predicates given in $J$, the data points in $\mathcal{S}^-$ don't satisfy their respective predicates in $J$, and for $x_1 \land  \dots \land x_n \rightarrow x \in C$, it is not the case that $x_1,\dots,x_n$ satisfy their respective predicates in $J$ while $x$ does not.

Finding a $J$ consistent with the sample $\mathcal{S}$
can be considered a \emph{classification problem} for $\mathcal{S}$.
We call such a $J$ a \emph{solution/classifier} of $\mathcal{S}$.
We say that a data point {\emph satisfies} $J$ iff it satisfies all its
associated predicates.

$J$ is not necessarily a solution of the CHC problem.
Hence, given a classifier $J$ provided by the \emph{learner}, the \emph{teacher} which knows the CHC system, checks in line~\ref{hornice:line:check}, if $J$ is indeed a solution for the system; If yes, a solution has been found and the process stops; otherwise a counterexample is given to update the sample for the next iteration, in line~\ref{hornice:line:addce}.
To check that $J$ is a solution,
the teacher considers the satisfiability of each clause by inserting
for each predicate in $\mathcal{P}$ the formula given by $J$.
If a clause $\forall \vec{v}.\; \phi(\vec{v}) \implies \Predicate{P_j}(\vec{v})$ is violated a counterexample is generated which is a data point $x$ associated with the predicate $\Predicate{P_j} \in \mathcal{P}$ together with a Horn implication $\top \rightarrow x$, meaning that $x$ must be satisfied by
$\Predicate{P_j}$.
If a clause $\forall \vec{v}_1,\dots,\vec{v}_n.\; \Predicate{P_1}(\vec{v}_1) \land \dots \land \Predicate{P_n}(\vec{v}_n) \land \phi(\vec{v}_1,\dots,\vec{v}_n) \implies \bot$ is violated, the counterexample is data points $x_1,\dots,x_n$ with Horn implication $x_1 \land \dots \land x_n \rightarrow \bot$, meaning that at least one of the $x_1,\dots,x_n$ must not satisfy its predicate.
If a clause $\forall \vec{v}_1,\dots,\vec{v}_n,\vec{v}.\; \Predicate{P_1}(\vec{v}_1) \land \dots \land \Predicate{P_n}(\vec{v}_n) \land \phi(\vec{v}_1,\dots,\vec{v}_n,\vec{v}) \implies \Predicate{P_j}(\vec{v})$ is violated, the counterexample is data points $x_1,\dots,x_n, x$ with Horn implication $x_1 \land \dots \land x_n \rightarrow x$. %, meaning that if all the data points $x_1,\dots,x_n$ satisfy their respective predicates, then $x$ must satisfy the predicate $\Predicate{P_j}$.
In all cases, the sample is updated to fulfill properties (\ref{eq:cs:1}-\ref{eq:cs:4}).
If the update results in a contradictory sample, i.e. $\mathcal{S}^+ \cap \mathcal{S}^- \neq \emptyset$, it means that the CHC system is unsatisfiable, and $\texttt{UNSAT}$ is returned.
It is worth noting that, in general, the Horn-ICE loop is not guaranteed to terminate and if the underlying logic is not decidable, the teacher might
not be able to answer.


==> quantified-horn-ice.tex <==
%\section{Learning Quantified Formulas with Horn-ICE}

%The instantiation of Horn-ICE for solving CHC over parametric-size arrays, necessitating quantified formulas as solutions for the unknown predicates, requires (1) a teacher capable of checking the validity of the clauses with the unknown predicates substituted with their candidate solution and (2) a learner able to synthesize quantified properties as classifiers
%for the Horn-ICE sample of counterexamples 
%provided in previous iterations by the teacher (these counterexamples
%contain parametric-size array constants).
%Hence, we implement the teacher using
%the SMT-solver Z3~\cite{z3} which can handle different
%decidable fragments of array logics~\cite{array-theory,erp-in-z3,arrays-in-z3}\footnote{In the literature arrays are typically
%handled using uninterpreted functions. We can easily encode parametric-size arrays
%like that.}.
%Z3 attempts to solve queries beyond the known decidable fragments using various heuristics.

%Decision trees are behind efficient instantiations of ICE~\cite{ice,boutglay22} and Horn-ICE~\cite{horn-ice}. However, they are restricted to numerical and boolean domains and it is not obvious how to use them for learning \emph{quantified} properties.
%In Section~\ref{sec:diagramization}, we propose a mechanism for reducing
%the classification problem of a Horn-ICE sample with parametric-size arrays to another classification problem where such arrays are transformed
%by introducing free variables.
%A quantifier-free formula can then be learned as a solution for this new problem using any classification method that can deal with Horn implications.
%We prove that quantifying the introduced free variables in such a solution results in a quantified solution for the original sample.
%Using these primitives, we build in Section~\ref{sec:qdt-learner} a decision-tree-based learner capable of synthesizing quantified properties.
%The example below illustrates the interaction between such a teacher and a learner.

%To instanciate Horn-ICE for solving CHC over parametric-size array theory $\BoundedArrayTheory{\BoundedArray}{E}$ derived from array-manipulating programs, as these CHC often requires quantified interpretations for their uninterpreted predicates, we need a learner that can infer quantified solutions (Section~\ref{section:qdt-learner}) and a teacher that can checks their validity. We provide the teacher with the decision procedure for the parametric-size array property fragment. It is important to note that to verify the validity of a CHC where every uninterpreted predicate is substituted with its interpretation from the candidate solution, it is sufficient to check the satisfiability of its negation. This falls within the decidable parametric-size array property fragment if the interpretations are parametric-size array properties. In the case of non-validity, the data point in the generated counterexample assigns a constant fixed-size array to every array variable in the domain of the predicate associated with this data point.

%\begin{example}
%Continuing with bubble sort from Example~\ref{example:bubble-sort}, we illustrate the interaction between the teacher and the learner to solve the CHC derived for this program.
%Initially with empty sample, the learner
%just proposes that both $\Predicate{I_0}$ and $\Predicate{I_1}$ are $true$.
%The teacher provides the counterexample $\langle \Predicate{I_0}, N \mapsto 2, a \mapsto [1, 0], s \mapsto \bot \rangle \rightarrow \bot$, i.e.
%$\langle \Predicate{I_0}, N \mapsto 2, a \mapsto [1, 0], s \mapsto \bot \rangle$ should not satisfy the learners hypothesis for $\Predicate{I_0}$, as this state violates the assertion in line~\ref{bsx:line:assert}.
%The learner then proposes $\Predicate{I_0}$ to be $\forall k_1,k_2.\; 0 \leq k_1 \leq k_2 < \BoundedArrayLength{a} \implies a[k_1] > 0$, while $\Predicate{I_1}$ remains $true$.
%The teacher gives back the counterexample $\top \rightarrow \langle \Predicate{I_0}, N \mapsto 1, a \mapsto [0], s \mapsto \top \rangle$, indicating that $\langle \Predicate{I_0}, N \mapsto 1, a \mapsto [0], s \mapsto \top \rangle$ should
%satisfy the next hypothesis for $\Predicate{I_0}$.
%Several iterations later, %precisely at the 10th iteration,
%the learner has accumulated more counterexamples depicted in the sample in Fig.~\ref{fig:data-sample} where variables names are omitted.
%Here the learner proposes $\forall k_1, k_2.\; 0 \leq k_1 \leq k_2 < \BoundedArrayLength{a} \implies a[k_1] \leq a[k_2] \lor s$ for $\Predicate{I_0}$ and $\forall k_1, k_2.\; 0 \leq k_1 \leq k_2 < \BoundedArrayLength{a} \implies a[k_1] \leq a[k_2] \lor i \leq k_2 \lor s$ for $\Predicate{I_1}$.
%However, the invariants are still not inductive and the teacher gives back the counterexample $\langle \Predicate{I_1}, N \mapsto 3, a \mapsto[1,1,0], i \mapsto 2, s \mapsto \bot \rangle \rightarrow \langle \Predicate{I_1}, N \mapsto 3, a \mapsto [1,0,1], i \mapsto 3, s \mapsto \top \rangle$.
%The learner finally guesses $\forall k_1,k_2.\; 0 \leq k_1 \leq k_2 < \BoundedArrayLength{a} \implies a[k_1] \leq a[k_2] \lor s$ %\footnote{Equivalent to $\forall k_1,k_2.\; 0 \leq k_1 \leq k_2 < \BoundedArrayLength{a} \land \neg s \implies a[k_1] \leq a[k_2]$}
%for $\Predicate{I_0}$, which states that if no swapping has been performed on the array ($\neg s$), then it is sorted, and for $\Predicate{I_1}$ it proposes
%$\forall k_1,k_2.\; 0 \leq k_1 \leq k_2 < \BoundedArrayLength{a} \implies a[k_1] \leq a[k_2] \lor i \leq k_2 \lor s$. %\footnote{Equivalent to $\forall k_1,k_2.\; 0 \leq k_1 \leq k_2 < \BoundedArrayLength{a} \land k_2 < i \land \neg s \implies a[k_1] \leq a[k_2]$}.
% The teacher confirms these to be adequate inductive invariants, thus the program is safe.
%\iflong
%Appendix~\ref{appendix:bubble-sort-iterations} provides more details.
%\else
%Appendix~B of the extended version of this paper in the supplementary material provides more details.
%\fi
% %illustrates the complete interaction between the learner and the teacher, with the omitted iterations in this example).
%\end{example}


==> unused-bounded-array-theory.tex <==
\subsection{Bounded-Size Array Theory}
\label{subsec:parametric-size-array-theory}

\begin{definition}[Bounded-Size Array Property]
A \emph{parametric-size array property} is a formula of the form
\begin{equation}
\forall \overrightarrow{Q_{a_1}}, \dots ,\overrightarrow{Q_{a_n}} .\; \big(\bigwedge\limits_{i=1}^n \QuantifierGuard{\overrightarrow{Q_{a_i}}}\big) \land G(\overrightarrow{Q_{a_1}}, \dots ,\overrightarrow{Q_{a_n}}) \implies D(\overrightarrow{Q_{a_1}}, \dots ,\overrightarrow{Q_{a_n}})
\end{equation}
where \begin{itemize}
\item $\overrightarrow{Q_{a_i}}$ is a set of quantified index variables used to access/read from the array $a_i$.
\item $\mathcal{G}(\overrightarrow{Q_{a}})$ denotes the boolean predicate
\begin{equation}
\mathcal{G}(\overrightarrow{Q_{a}}) = \bigwedge\limits_{k \in \overrightarrow{Q_{a}}} 0 \leq k < |a|
\end{equation}
\item $G(\overrightarrow{Q_{a_1}}, \dots ,\overrightarrow{Q_{a_n}})$
  is an index guard...
\item $D(\overrightarrow{Q_{a_1}}, \dots ,\overrightarrow{Q_{a_n}})$
  is a value constraint...
\end{itemize}

The form of $G(\overrightarrow{Q_{a_1}}, \dots ,\overrightarrow{Q_{a_n}})$ is restricted according to the following grammar:
\begin{grammar}\centering
<guard> ::= <guard> $\land$ <guard> | <guard> $\lor$ <guard> | <iatom>

<iatom> ::= <iexpr> $\leq$ <iexpr> | <iexpr> = <iexpr>

<iexpr> ::= uvar | "|"eavar"|" | <piexpr>

<piexpr> ::= $\Z$ | $\Z$.evar | <piexpr> + <piexpr>
\end{grammar}
and the form $D(\overrightarrow{Q_{a_1}}, \dots ,\overrightarrow{Q_{a_n}})$ is restricted according to the following grammar:
\begin{grammar}\centering
<constaint> ::= <constaint> $\land$ <constaint> | <constaint> $\lor$ <constaint> | <gatom>

<gatom> ::= <gexpr> $\leq$ <gexpr> | <gexpr> = <gexpr>

<gexpr> ::= $\Z$ | $\Z$.evar | eavar[<iexpr>] | <gexpr> + <gexpr>
\end{grammar}
where $uvar \in \bigcup_{i=1}^{n} \overrightarrow{Q_{a_n}}$ is a an universally quantified variable, $eavar$ is any existentially quantified parametric-size array variables and $evar$ is any existentially quantified integer variables. We additionally impose that the intersection of the existentially quantified integer variables evar appearing in $\langle piexpr\rangle$ and those in $\langle gexpr\rangle$ is empty.
\end{definition}

\begin{definition}
\label{def:bounded-array-property-fragment}
We call the set of all existentially-closed boolean combinations of parametric-size array property formulae and quantifier-free $\BoundedArrayTheory{\BoundedArray}{E}$-formulae, the \emph{parametric-size array property fragment}.
\end{definition}

\begin{theorem}
Satisfiability of a formula in parametric-size array property fragment is decidable.
\end{theorem}
\begin{proof} % precise this proof
Let $\phi$ be a formula belonging to the parametric-size array property fragment. For each parametric-size array $a$ occurring in $\phi$, we introduce a fresh (unbounded) array denoted by $u_a$, as well as a fresh integer variable represented by $l_a$. By performing the following substitutions throughout $\phi$:
\begin{itemize}
\item Substituting $\BoundedArrayLength{a}$ with $l_a$;
\item Substituting any atomic formula $t$ containing $\BoundedArrayRead{a}{i}$ with $ite(0 \leq i < l_a, t[\BoundedArrayRead{a}{i}/u_a[i]], false)$;
\item Substituting $\BoundedArrayWrite{a}{i}{v}$ with $ite(0 \leq i < l_a, u_a\{i\leftarrow v\}, u_a)$. % should we define "ite" it somewhere beforehand?
\end{itemize}
We obtain a formula $\phi'$ belonging to the decidable array property fragment, as presented in \cite{array-theory}.
By using the decision procedure of \cite{array-theory} on the transformed formula $\phi'$
\begin{itemize}
\item If $\phi'$ is satisfiable then $\phi$ is also satisfiable; \\
We prove that, by contradiction. Let $\phi'$ be satisfiable and assume, for now, that $\phi$ is not satisfiable. This means that there exists no model with free index variables $i$ accessing/writing an array $a$ in $\phi$ with a value in the interval $\Interval{0}{|a| - 1}$. $\phi'$ following the substitution above must not have a model that assigns to the index variables values in $\Interval{0}{|a| - 1}$. This is contradictory with the fact that $\phi'$ is satisfiable as any model of it must assign a value in $\Interval{0}{|a| - 1}$ to the index variables otherwise $\phi$ would have been unsatisfiable.
\item If $\phi'$ is unsatisfiable then $\phi$ is also unsatisfiable; \\
This can be proven in a symmetric way to how we proved the previous case.
\end{itemize}
\end{proof}

